Boosting Redundancy-based Automated Program Repair by Fine-grained Pattern Mining

Redundancy-based automated program repair (APR), which generates patches by referencing existing source code, has gained much attention since they are effective in repairing real-world bugs with good interpretability. However, since existing approaches either demand the existence of multi-line similar code or randomly reference existing code, they can only repair a small number of bugs with many incorrect patches, hindering their wide application in practice. In this work, we aim to improve the effectiveness of redundancy-based APRs by exploring more effective source code reuse methods for improving the number of correct patches and reducing incorrect patches. Specifically, we have proposed a new repair technique named Repatt, which incorporates a two-level pattern mining process for guiding effective patch generation (i.e., token and expression levels). We have conducted an extensive experiment on the widely-used Defects4J benchmark and compared Repatt with ten state-of-the-art APR approaches. The results show that it complements existing approaches by repairing 9 unique bugs compared with the latest Large Language Model (LLM)-based and deep learning-based methods and 19 unique bugs compared with traditional repair methods when providing the perfect fault localization. In addition, when the perfect fault localization is unknown in real practice, Repatt significantly outperforms the baseline approaches by achieving much higher patch precision, i.e., 83.8\%, although it repairs fewer bugs. Moreover, we further proposed an effective patch ranking strategy for combining the strength of Repatt and the baseline methods. The result shows that it repairs 124 bugs when only considering the Top-1 patches and improves the best-performing repair method by repairing 39 more bugs. The results demonstrate the effectiveness of our approach for practical use.

==> algo/abstraction.tex <==
\begin{algorithm}[t]
	\small
	\caption{Adaptive Code Element Abstraction}
	\label{alg:abstract}
	\SetKwInput{KwInput}{Input}                % Set the Input
	\SetKwInput{KwOutput}{Output}              % set the Output
	\DontPrintSemicolon
	
	\KwInput{\textit{freqMap:} \textcolor{gray}{a map of program elements and their frequencies.} 
	\textit{method:} \textcolor{gray}{a method to be embedded.}}
	\KwOutput{\textit{ES:} \textcolor{gray}{a sequence of the element embeddings (IDs).}}
	%	\KwData{}
	
	% Set Function Names
	\SetKwFunction{FMain}{codeAbstraction}
	\SetKwFunction{FBuild}{embedElement}
	
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FMain{\textit{freqMap, method}}}{
		\textit{ES} $\leftarrow  []$ \;
		\textit{stmts} $\leftarrow$ statements in \textit{method}\;
		\ForEach{s in stmts}{
			\textit{ids} $\leftarrow$ \FBuild{freqMap, s}\;
			\textit{ES.append(ids)}\;
		}
		\KwRet \textit{ES}
	}
	\Fn{\FBuild{\textit{freqMap, elem}}}{
		\textit{S} $\leftarrow []$\;
		\textit{freq} $\leftarrow$ \textit{freqMap.get(elem)}\;
		\uIf{freq $\ge$ threshold or elem is a leaf node}{
			\textit{id} $\leftarrow$ \textit{EMBEDDING.getOrInsert(elem)}\;
			\textit{S.append(id)}
		}
		\Else{
			\ForEach{child node e of s}{
				S.append(\FBuild{freqMap, e})\;
			}
		}
		\KwRet \textit{S}
	}
\end{algorithm}


==> algo/encoding.tex <==
\begin{algorithm}
	\caption{Adaptive encoding algorithm} \label{alg:cap}
	\begin{algorithmic}
		\Require a number sequence S
		\Ensure a codeBlock
		\State Statements $\gets$ split(statement, codeBlock)
		\For {each stmt in Statements}
		\If{isFrequent(stmt)}
		\State S.add(getFrequentId(stmt))
		\ElsIf{Expressions $\gets$ split(expression,stmt)}
		\For{each exp in Expressions}
		\If{isFrequent(exp)}
		\State S.add(getFrequentId(exp))
		\ElsIf{Tokens $\gets$ split(token,exp)}
		\For{each token in Tokens}
		\If{isFrequent(token)}
		\State S.add(getFrequentId(token))
		\EndIf
		\EndFor
		\EndIf
		\EndFor
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}

==> algo/match.tex <==
\begin{algorithm}
	\caption{Similar pattern mining algorithm} \label{alg:cap}
	\begin{algorithmic}
		\Require prefix-tree T
		\Ensure similar pattern set S
		\Function{dfs}{sequence}
		\If{node has no child nodes with at least MIN\_SUPPORT occurrence}
		\If{calculateSimilarity(sequence,targetSequence) $\ge$ SIMILARITY}
		\State put sequence into S
		\EndIf
		\Else
		\For{child node N}
		\If{N.count $\ge$ MIN\_SUPPORT}
		\State put N into sequence
		\State dfs(sequence)
		\EndIf
		\EndFor
		\EndIf
		\EndFunction
	\end{algorithmic}
\end{algorithm}

==> algo/sequence.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
	\caption{Sequence generating algorithm} \label{alg:cap}
	\begin{algorithmic}
		\Require sequence $N_1N_2\ldots N_m$
		\Ensure sub-sequence set S
		\Function{seq}{start, length, skip, state}
		\If{length = 0}
		\State put state into S
		\ElsIf{start $<$ $m$}
		\State copy $\gets$ state + $N_{start}$
		\State SEQ(start+1, length-1, 0, copy)
		\If{skip $<$ MAX\_SKIP}
		\State SEQ(start+1, length, skip+1, state)
		\EndIf
		\EndIf
		\EndFunction
	\end{algorithmic}
\end{algorithm}
% \begin{algorithm}
	% \caption{Sequence generating algorithm} \label{alg:cap}
	% \begin{algorithmic}
		% \Require sequence $N_1N_2\ldots N_m$
		% \Ensure sub-sequence set S
		% \For {each sequence $N_1N_2 \ldots N_m$ in S}
		%     \State cur $\gets$ root
		%     \For {each char c in sequence}
		%         \If{cur has children c}
		%             \State cur.children[c].count += 1
		%             \State cur $\gets$ cur.children[c]
		%         \Else
		%             \State cur.children[c] $\gets$ new node(c)
		%             \State cur.children[c].count $\gets$ 1
		%             \State cur $\gets$ cur.children[c]
		%         \EndIf
		%     \EndFor
		% \EndFor
		% \end{algorithmic}
	% \end{algorithm}

==> code/JacksonDatabind_82.tex <==
% \noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[ style=Java,caption=Patch code of JacksonDatabind-82 in Defects4J,label=lst:JD82] 
<@\lin{493}@>    builder.setIgnoreUnknownProperties(ignoreAny);
<@\lin{494}@>    // Or explicit/implicit definitions?
<@\hlc{red!15}{\lin{495}\quad-\quad   ignored = ignorals.getIgnored();}    @>
<@\hlc{green!15}{\quad\ \ \  +\quad ignored = ignorals.findIgnoredForDeserialization(); }@>
<@\lin{496}@>    for (String propName : ignored) {
<@\lin{497}@>        builder.addIgnorable(propName);...
\end{lstlisting}
% \end{minipage}
% \vspace{-8pt}
% \begin{lstlisting}[ style=Java,caption=Patch code of Gson-17 in Defects4J,label=lst:gson17] 
% <@\lin{98}@>    public Date read(JsonReader in) throws IOException {
% <@\hlc{red!15}{\lin{99}\quad  -\qquad   if (in.peek() != JsonToken.STRING) \{}    @>
% <@\hlc{red!15}{\lin{100} -  \qquad\qquad throw new JsonParseException("The date ...");}@>
% <@\hlc{green!15}{\qquad +\qquad   if (in.peek() == JsonToken.NULL) \{ }@>
% <@\hlc{green!15}{\qquad + \qquad\qquad  in.nextNull(); }@>
% <@\hlc{green!15}{\qquad +  \qquad\qquad   return null; }@>
% <@\lin{101}@>     }
% <@\lin{102}@>     Date date = deserializeToDate(in.nextString()); ...
% \end{lstlisting}

% \begin{lstlisting}[ style=Java,caption=Patch code of Codec-3 in Defects4J,label=lst:codec3] 
% <@\lin{452}@>   if ((contains(value, 0 ,4, "VAN ", "VON ") || ...)){
% <@\lin{453}@>       //-- obvious germanic --//;
% <@\lin{454}@>       result.append('K');
% <@\hlc{red!15}{\lin{455} - \} else if(contains(value, index + 1, 4, "IER")) \{}@>
% <@\hlc{green!15}{\qquad   + \} else if(contains(value, index + 1, 3, "IER")) \{}@>
% <@\lin{456}@>       result.append('J');
% <@\lin{457}@>  } else {...
% \end{lstlisting}
% % \vspace{-8pt}

==> code/JacksonDatabind_82_donor.tex <==
\begin{lstlisting}[ style=Java,caption=The reference code for repairing JacksonDatabind-82,label=lst:JD82Donor] 
<@\lin{1}@>    JsonIgnoreProperties.Value ignorals=intr.findPropertyIgnorals(accessor);
<@\lin{2}@>    if (ignorals != null) {
<@\lin{3}@>        ignoredProps = ignorals.findIgnoredForDeserialization();
<@\lin{4}@>    }
<@\lin{5}@>    ObjectIdInfo objectIdInfo = intr.findObjectIdInfo(accessor);
\end{lstlisting}

==> code/cli17.tex <==
\begin{lstlisting}[ style=Java,caption=Patch code of Time-7 in Defects4J,label=lst:time7] 
<@\lin{707}@>  Chronology chrono = instant.getChronology();
<@\lin{708}@>  long instantLocal = instantMillis + chrono.getZone().getOffset(instantMillis);
<@\hlc{red!15}{\lin{709}- int defaultYear = chrono.year().get(instantLocal);}@>
<@\hlc{green!15}{\qquad  + int defaultYear = chrono.year().get(instantMillis);}@>

<@\lin{300}@>else if (stopAtNonOption)
<@\lin{301}@>{
<@\lin{302}@>           process(token.substring(i));
<@\lin{303}@>
<@\lin{304}@>
<@\lin{305}@>
\end{lstlisting}

==> code/gson15.tex <==
% \noindent\begin{minipage}{\linewidth}


% \begin{lstlisting}[style=Java,caption=Patch code of Gson-15 in Defects4J,label=lst:GS15] 
% <@\lin{493}@>    public JsonWriter value(double value) throws IOException {
% <@\lin{494}@>        writeDeferredName();
% <@\hlc{red!15}{\lin{495}\qquad  -\qquad \  if (Double.isNaN(value) || Double.isInfinite(value)) \{}    @>
% <@\hlc{red!15}{\lin{496}\qquad  -\qquad \ \qquad  throw new IllegalArgumentException("Numeric values must be finite, but was " + value);}    @>
% <@\hlc{red!15}{\lin{497}\qquad  -\qquad \  \}}    @>
% <@\hlc{green!15}{\qquad\ \ \  +\quad\ \ \ if (!lenient) }@>
% <@\hlc{green!15}{\qquad\ \ \  +\quad\ \ \ \ \qquad if (Double.isNaN(value) || Double.isInfinite(value)) \{ }@>
% <@\hlc{green!15}{\qquad\ \ \  +\quad\ \ \ \ \qquad \qquad throw new IllegalArgumentException("Numeric values must be finite, but was " + value); }@>
% <@\hlc{green!15}{\qquad\ \ \  +\quad\ \ \ \ \qquad \}}@>
% <@\lin{498}@>         beforeValue();...
% \end{lstlisting}


\begin{lstlisting}[style=Java,caption=Patch code of Gson-15 in Defects4J,label=lst:gson15] 
<@\lin{494}@>   writeDeferredName();
<@\hlc{red!15}{\lin{495} - if(Double.isNaN(value) || Double.isInfinite(value))\{}    @>
<@\hlc{red!15}{\lin{496} - \qquad throw new IllegalArgumentException(...);}    @>
<@\hlc{red!15}{\lin{497} - \}}    @>
<@\hlc{green!15}{\phantom{497} + if (!lenient) }@>
<@\hlc{green!15}{\phantom{497} + \quad if(Double.isNaN(value)||Double.isInfinite(value))\{}@>
<@\hlc{green!15}{\phantom{497} + \qquad throw new IllegalArgumentException(...); }@>
<@\hlc{green!15}{\phantom{497} +\quad\}}@>
<@\lin{498}@>   beforeValue();...
\end{lstlisting}

==> code/gson15dornor.tex <==
% \noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[ style=Java,caption=The reference code for repairing Gson-15, label=lst:gson15donor] 
<@\lin{1}@>  JsonToken token=peek();
<@\lin{2}@>  if(token!=JsonToken.NUMBER && token!=JsonToken.STRING){
<@\lin{3}@>    throw new IllegalStateException(...);
<@\lin{4}@>  }
<@\lin{5}@>  if(!isLenient()
<@\lin{6}@>     &&(Double.isNaN(result)||Double.isInfinite(result))){
<@\lin{7}@>       throw new NumberFormatException(...);
<@\lin{8}@>  }
<@\lin{9}@>  popStack();...
\end{lstlisting}


==> fig/table/combine.tex <==
\begin{table}[!t]
\caption{Sources of correct patches}
	\label{tab:combine_sources}
\centering
\resizebox{\columnwidth}{!}{
\setlength\tabcolsep{3pt}
\begin{threeparttable}
\begin{tabular}{l|c|c|c|c|c}
\toprule
\bf{} & \bf{SimFix} & \bf{TBar} & \bf{TransplantFix} & \cellcolor{lightgray}\bf{\tool{}} \\
\midrule
Number     & 12           & 39        & 23           & \cellcolor{lightgray}\bf{39}           \\
Ratio (\%)     & 9.6            & 31.2          & 18.4   & \cellcolor{lightgray}\bf{40.8}      
\\ \bottomrule      
\end{tabular}
\end{threeparttable}
}
\end{table}

==> fig/table/comparePL.tex <==
\begin{table*}[!t]
\caption{Number of bugs repaired by different methods with perfect fault localization.
%	\hy{The results in Table 1 show that RePatt may not be the best?}
%	\jcom{@Zhirui, add the results of learning-based methods. If no enough space, we can report the overall results on D4J1.2 and D4J2.0. respectively.}
}	\label{tab:comparisonPerfect}
	\centering
	%\scriptsize
	\setlength\tabcolsep{3pt}
	\resizebox{1.00\textwidth}{!}
   {
    	\begin{threeparttable}
% 			\begin{tabular}{l|c|c|c|c|c}
% 			\toprule
% 		      {\bf Project} & {\bf  Recoder} &  {\bf  TBar} & {\bf SimFix}  & {\bf TransplantFix}   & {\cellcolor{lightgray}{\bf \tool{}}}  \\ 
% 	        \midrule
% Chart           & 10/-           & 11/13       & 8/16       & 6/10                 & \cellcolor{lightgray}{\bf 6/7}      \\
% Cli             & 3/-            & 1/7           & 0/1          & 4/8                 & \cellcolor{lightgray}{\bf 3/9}      \\
% Closure         & 23/-           & 17/25       & 7/15       & 10/22                & \cellcolor{lightgray}{\bf 11/12}    \\
% Codec           & 2/-            & 3/6         & 1/1          & 2/4                 & \cellcolor{lightgray}{\bf 3/6}      \\
% Collections     & 0/-            & 0/0           & 0/0          & 0/0                 & \cellcolor{lightgray}{\bf 0/0}      \\
% Compress        & 3/-            & 2/12           & 0/4          & 4/10                 & \cellcolor{lightgray}{\bf 3/13}     \\
% Csv             & 4/-            & 3/6           & 0/2          & 1/2                 & \cellcolor{lightgray}{\bf 1/3}      \\
% Gson            & 0/-            & 1/4           & 2/2          & 1/2                 & \cellcolor{lightgray}{\bf 2/3}      \\
% JacksonCore     & 0/-            & 0/5           & 0/2          & 1/6                 & \cellcolor{lightgray}{\bf 2/7}      \\
% JacksonDatabind & 0/-            & 2/17           & 1/10          & 7/20                 & \cellcolor{lightgray}{\bf 10/18}    \\
% JacksonXml      & -              & 0/1           & 0/0          & 0/0                 & \cellcolor{lightgray}{\bf 0/0}      \\
% Jsoup           & 7/-            & 7/17           & 1/2          & 3/8                 & \cellcolor{lightgray}{\bf 3/13}     \\
% JxPath          & 0/-            & 0/0           & 0/0          & 2/7                 & \cellcolor{lightgray}{\bf 0/5}      \\
% Lang            & 10/-           & 13/18       & 8/15       & 4/10                & \cellcolor{lightgray}{\bf 6/11}     \\
% Math            & 19/-           & 22/34       & 20/33      & 12/25                & \cellcolor{lightgray}{\bf 14/25}    \\
% Mockito         & 2/-            & 3/3         & 1/2        & 3/3                 & \cellcolor{lightgray}{\bf 1/2}      \\
% Time            & 3/-            & 2/5         & 3/6        & 1/3                 & \cellcolor{lightgray}{\bf 1/3}      \\ \midrule
% Total           & 66/-           & 87/173       & 52/111      & 61/140                & \cellcolor{lightgray}{\bf 66/136}   \\ \midrule
% P(\%)           & -              & 50.3        & 46.8       & 43.6                   & \cellcolor{lightgray}{48.5}         \\ 
% 		\bottomrule
% 		\end{tabular}
\begin{tabular}{cl|c|c|c|c|c|c|c|c|c|c}
\toprule
&  {\bf Project} & {\bf  Recoder}     &{\bf  TBar}    &{\bf SimFix}  & {\bf TransplantFix}   & {\bf SelfRepair} & {\bf CodeT5} & {\bf CodeGen} & {\bf PLBART} &  {\cellcolor{lightgray}{\bf \tool{}}} &  {\cellcolor{lightgray}{\bf \combine{}}}\\
 \midrule
 \multirow{6}{*}{\makecell{Defects4J v1.2 \\ (395 bugs)}} &
  Mockito          & 2/-              & 3/3           & 0/0     & 3/3       & 3/3       & 4/5       & 3/4       & 2/3    & \cellcolor{lightgray}{\bf 1/2}       & \cellcolor{lightgray}{\bf 2/5} \\
& Closure          & 23/-             & 16/24         & 5/6     & 10/19     & 19/23     & 6/9       & 9/12      & 4/10   & \cellcolor{lightgray}{\bf 10/12}     & \cellcolor{lightgray}{\bf 20/31} \\
& Chart            & 10/-             & 11/13         & 4/8     & 6/10      & 7/10      & 4/4       & 7/7       & 4/4    & \cellcolor{lightgray}{\bf 6/7}       & \cellcolor{lightgray}{\bf 11/21} \\
& Lang             & 10/-             & 13/18         & 8/13    & 4/10      & 10/13     & 6/8       & 5/5       & 4/4    & \cellcolor{lightgray}{\bf 6/11}      & \cellcolor{lightgray}{\bf 16/27} \\
& Math             & 18/-             & 22/35         & 14/26   & 12/25     & 21/25     & 12/14     & 12/14     & 13/16  & \cellcolor{lightgray}{\bf 15/25}     & \cellcolor{lightgray}{\bf 22/51} \\
& Time             & 3/-              & 3/6           & 1/1     & 1/2       & 3/3       & 1/1       & 2/2       & 2/2    & \cellcolor{lightgray}{\bf 2/3}       & \cellcolor{lightgray}{\bf 4/7} \\ 
\midrule \multirow{12}{*}{\makecell{Defects4J v2.0\\ (440 bugs)}} 
& Closure          & 0/-              & 0/0           & 1/1     & 0/3       & 1/1       &1/1        & 1/1       &1/1     & \cellcolor{lightgray}{\bf 1/1}       & \cellcolor{lightgray}{\bf 2/5} \\
& Cli              & 3/-              & 1/7           & 0/1     & 4/8       & 8/9       & 2/3       & 4/5       & 2/3    & \cellcolor{lightgray}{\bf 4/9}       & \cellcolor{lightgray}{\bf 4/15} \\
& Codec            & 2/-              & 3/6           & 1/1     & 2/4       & 8/9       & 1/1       & 2/3       & 1/1    & \cellcolor{lightgray}{\bf 4/6}       & \cellcolor{lightgray}{\bf 3/8} \\
& Collections      & 0/-              & 0/0           & 0/0     & 0/0       & 1/1       & 0/0       & 1/1       & 0/0    & \cellcolor{lightgray}{\bf 0/0}       & \cellcolor{lightgray}{\bf 0/0} \\
& Compress         & 3/-              & 2/12          & 0/4     & 4/10      & 6/8       & 3/5       & 3/6       & 3/5    & \cellcolor{lightgray}{\bf 4/13}      & \cellcolor{lightgray}{\bf 7/18} \\
& Csv              & 3/-              & 2/6           & 0/2     & 1/2       & 1/1       & 1/2       & 2/3       & 2/4    & \cellcolor{lightgray}{\bf 1/3}       & \cellcolor{lightgray}{\bf 2/7} \\
& Gson             & 0/-              & 1/4           & 2/2     & 1/2       & 1/1       & 0/0       & 0/0       & 0/0    & \cellcolor{lightgray}{\bf 2/3}       & \cellcolor{lightgray}{\bf 2/5} \\
& JacksonCore      & 0/-              & 0/5           & 0/2     & 1/6       & 3/3       & 3/3       & 2/3       & 2/2    & \cellcolor{lightgray}{\bf 3/7}       & \cellcolor{lightgray}{\bf 3/9} \\
& JacksonDatabind  & 0/-              & 2/17          & 1/10    & 7/20      & 8/10      & 4/7       & 3/6       & 2/4    & \cellcolor{lightgray}{\bf 10/18}     & \cellcolor{lightgray}{\bf 11/33} \\
& JacksonXml       & -                & 0/1           & 0/0     & 0/0       & 1/1       &0/0        & 0/0       & 0/0    & \cellcolor{lightgray}{\bf 0/0}       & \cellcolor{lightgray}{\bf 1/1} \\
& Jsoup            & 7/-              & 6/17          & 1/2     & 3/8       & 6/8       & 4/6       & 5/7       & 4/5    & \cellcolor{lightgray}{\bf 5/13}      & \cellcolor{lightgray}{\bf 10/25} \\
& JxPath           & 0/-              & 1/6           & 0/0     & 2/7       & 1/1       & 0/0       & 0/1       & 0/1    &  \cellcolor{lightgray}{\bf 1/5}      & \cellcolor{lightgray}{\bf 4/12} \\ 
\midrule
\multicolumn{2}{c|}{Total}       
                   &84/-             &  85/180        &  38/79  & 61/139    & 108/130   & 52/ 69    & 61/80     & 46/ 65 & \cellcolor{lightgray}{\bf 75/138 }   & \cellcolor{lightgray}{\bf 124/280}  \\ \midrule
\multicolumn{2}{c|}{Precision(\%) }          
                   & -               &  47.2          & 48.1    & 43.9      & 83.1      & 75.4      & 76.3      & 70.8   & \cellcolor{lightgray}{\bf 54.3}      & \cellcolor{lightgray}{\bf 44.3}\\
\bottomrule
\end{tabular}
% \begin{tablenotes}
%     \item[*] SelfRepair did consider the ranking of patches.
% \end{tablenotes}	
  \end{threeparttable}
}
\end{table*}

==> fig/table/component.tex <==
% \begin{table*}[!t]
% \caption{Number of bugs fixed by each component.}
% 	\label{tab:component}
% 	\centering
% 	%\scriptsize
% 	\setlength\tabcolsep{3pt}
% %	\resizebox{1.00\linewidth}{!}
% %    {
%     	\begin{threeparttable}
% 			\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% 			\toprule
% 		      {\bf Project} & {\bf Chart} & {\bf Gson} & {\bf  Csv}  & {\bf  Closure} & {\bf Codec} & {\bf Collections} & {\bf Compress}  &{\bf JacksonDatabind } & {\bf Lang }   \\ 
% 	        \midrule
%          Token-level pattern mining                & 5/6  & 0/0  & 0/0  & 10/10  & 3/5  & 0/0 & 2/6 & 5/9 & 2/4 \\
%          Expression-level code search              & 1/2  & 2/3  & 1/3  & 1/3    & 1/2  & 0/0 & 2/8 & 5/11 & 4/8 \\
%          \midrule\midrule
% 		      {\bf Project} & {\bf Math} & {\bf Time} & {\bf Cli}  & {\bf  Jsoup} & {\bf JxPath} & {\bf  JacksonXml} & {\bf  Mockito}  &  {\bf  JacksonCore} & {\bf Total}  \\ 
% 	        \midrule
%           Token-level pattern mining                & 10/15  & 2/3  & 0/2  & 1/2  & 0/0  & 0/0 & 1/1 & 1/1 & 42/64 \\
%           Expression-level code search              & 5/12  & 0/1  & 4/9  & 4/11  & 1/5  & 0/0 & 0/1 & 2/6 & 33/85 \\
% 		\bottomrule
% 		\end{tabular}
	
% 		\end{threeparttable}
% %	}
% \end{table*}

\begin{table}[!t]
\caption{Number of bugs fixed by each component.}
	\label{tab:component}
	\centering
\setlength\tabcolsep{3pt}
	\resizebox{0.98\columnwidth}{!}{
\begin{threeparttable}
\begin{tabular}{l|c|c||c|c}
\toprule
\textbf{Components} & Offline Mining & Online Search & No Skip & No S-TAC \\ \midrule
\textbf{Total}    & 42/64                         & 33/85         & 24/54            & 0/22  \\  
\textbf{Precision (\%)}    & 65.6                         & 38.8        &   44.4          & 0    
\\ \bottomrule     
\end{tabular}
\end{threeparttable}}
\end{table}



==> fig/table/deprecated.tex <==
\begin{table}[!t]
	\centering
	%\scriptsize
	\setlength\tabcolsep{2pt}
%	\caption{Comparing \toolname against the state-of-the-art APR tools.}
	\label{tab:comparisonPerfect}
%	\resizebox{1.00\linewidth}{!}
%    {
    	\begin{threeparttable}
% 			\begin{tabular}{l|c|c|c|c|c}
% 			\toprule
% 		      {\bf Project} & {\bf  Recoder} &  {\bf  TBar} & {\bf SimFix}  & {\bf TransplantFix}   & {\cellcolor{lightgray}{\bf Repatt}}  \\ 
% 	        \hline
%  Chart          & 8/14  & 9/14  & 4/8  & 8/16    & \cellcolor{lightgray}{\bf 9/14}\\
%  Cli            & 3/3  & 1/7  & 0/4    & -        & \cellcolor{lightgray}{\bf 9/14}\\
%  Closure        & 17/38 & 8/17 & 7/13  & 7/11   & \cellcolor{lightgray}{\bf 9/14}\\
%  Codec          & 2/2  & 2/6  & 0/2     & -     & \cellcolor{lightgray}{\bf 9/14}\\
%  Collections    & 0/0  & 0/1  & 0/1     & -    & \cellcolor{lightgray}{\bf 9/14}\\
%  Compress       & 3/9  & 1/13  & 0/6    & -    & \cellcolor{lightgray}{\bf 9/14}\\
%  Csv            & 4/4  & 1/5  & 0/2    & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  Gson           & -    & -     & -     & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  JacksonCore    & 0/4  &  0/6  & 0/0    & -     & \cellcolor{lightgray}{\bf 9/14}\\
%  JacksonDatabind& 0/0  & 0/0  & 0/0    & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  JacksonXml     & -    & -    & -      & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  Jsoup          & 7/13  & 3/7  & 1/5  & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  JxPath         & 0/4  & 0/0  & 0/0    &-      & \cellcolor{lightgray}{\bf 9/14}\\
%  Lang           & 9/15  & 5/14  & 9/13   & 8/15   & \cellcolor{lightgray}{\bf 9/14}\\
%  Math          & 15/30 & 18/36  & 14/26  & 20/41   & \cellcolor{lightgray}{\bf 9/14}\\
%  Mockito        & 2/2  & 1/2  & 0/0   & 1/2   & \cellcolor{lightgray}{\bf 9/14}\\
%  Time           & 2/2  & 1/3  & 1/1   & 3/6   & \cellcolor{lightgray}{\bf 9/14}\\
% 			\hline
% 	  Total   & 69/137  & 50/131  & 36/81  & 47/91   & \cellcolor{lightgray}{\bf 9/14} \\\hline
% P(\%)         & 50.4  & 38.2     & 44.4  & 51.6      & \cellcolor{lightgray}{11.1} \\
% 		\bottomrule
% 		\end{tabular}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\bf Project & \bf Recoder & \bf TBar & \bf SimFix & \bf TransplantFix & \bf SelfRepair & \bf CodeT5 & \bf CodeGen & \bf PLBART & \bf Repatt \\
Cli              & 3/-              & 1/7           & 0/1             & 4/8                    & 8/-                 & 2/3             & 4/5              & 2/3             & \cellcolor{lightgray}{\bf 3/9} \\
Codec            & 2/-              & 3/6           & 1/1             & 2/4                    & 8/-                 & 1/1             & 2/3              & 1/1             & \cellcolor{lightgray}{\bf 3/6} \\
Collections      & 0/-              & 0/0           & 0/0             & 0/0                    & 1/-                 & 0/0             & 1/1              & 0/0             & \cellcolor{lightgray}{\bf 0/0} \\
Compress         & 3/-              & 2/12          & 0/4             & 4/10                   & 7/-                 & 3/5             & 3/6              & 3/5             & \cellcolor{lightgray}{\bf 3/13}   \\
Csv              & 4/-              & 3/6           & 0/2             & 1/2                    & 1/-                 & 1/2             & 2/3              & 2/4             & \cellcolor{lightgray}{\bf 1/3} \\
Gson             & 0/-              & 1/4           & 2/2             & 1/2                    & 1/-                 & 0/0             & 0/0              & 0/0             & \cellcolor{lightgray}{\bf 2/3} \\
JacksonCore      & 0/-              & 0/5           & 0/2             & 1/6                    & 3/-                 & 3/3             & 2/3              & 2/2             & \cellcolor{lightgray}{\bf 2/7} \\
JacksonDatabind  & 0/-              & 2/17          & 1/10            & 7/20                   & 8/-                 & 4/7             & 3/6              & 2/4             & \cellcolor{lightgray}{\bf 10/18}  \\
JacksonXml       & -                & 0/1           & 0/0             & 0/0                    & 1/-                 & 0/0             & 0/0              & 0/0             & \cellcolor{lightgray}{\bf 0/0} \\
Jsoup            & 7/-              & 7/17          & 1/2             & 3/8                    & 6/-                 & 4/6             & 5/7              & 4/5             & \cellcolor{lightgray}{\bf 3/13}   \\
JxPath           & 0/-              & 0/0           & 0/0             & 2/7                    & 1/-                 & 0/0             & 0/1              & 0/1             & \cellcolor{lightgray}{\bf 0/5} \\
Mockito          & 2/-              & 3/3           & 1/2             & 3/3                    & 3/-                 & 4/5             & 3/4              & 2/3             & \cellcolor{lightgray}{\bf 1/2} \\
Closure          & 23/-             & 17/25         & 7/15            & 10/22                  & 20/-                & 7/10            & 10/13            & 6/11            & \cellcolor{lightgray}{\bf 11/12}  \\
Chart            & 10/-             & 11/13         & 8/16            & 6/10                   & 7/-                 & 4/4             & 7/7              & 4/4             & \cellcolor{lightgray}{\bf 6/7} \\
Lang             & 10/-             & 13/18         & 8/15            & 4/10                   & 10/-                & 6/8             & 5/5              & 4/4             & \cellcolor{lightgray}{\bf 6/11}   \\
Math             & 19/-             & 22/34         & 20/33           & 12/25                  & 21/-                & 12/14           & 12/14            & 13/16           & \cellcolor{lightgray}{\bf 14/25}  \\
Time             & 3/-              & 2/5           & 3/6             & 1/3                    & 3/-                 & 1/1             & 2/2              & 2/2             & \cellcolor{lightgray}{\bf 1/3} \\
Total            &                  &               &                 &                        &                     &                 &                  &                 & \cellcolor{lightgray}{\bf }       \\
P(\%)            &                  &               &                 &                        &                     &                 &                  &                 & \cellcolor{lightgray}{\bf }      
\end{tabular}
		\end{threeparttable}


\end{table}

==> fig/table/frequency.tex <==
% \begin{table*}[!t]
% \caption{Effects of Token-level fix with different frequent threshold\jcom{@Zijie, add frequency:5.}}
% 	\label{tab:frequency}
% 	\centering
% 	%\scriptsize
% 	\setlength\tabcolsep{3pt}
% %	\resizebox{1.00\linewidth}{!}
% %    {
%     	\begin{threeparttable}
% 			\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% 			\toprule
% 		      {\bf Project} & {\bf Chart} & {\bf Gson} & {\bf  Csv}  & {\bf  Closure} & {\bf Codec} & {\bf Collections} & {\bf Compress}  &{\bf JacksonDatabind } & {\bf Lang }   \\ 
% 	        \midrule
%          Frequency:2      & 6/8  & 0/0  & 0/1  & 10/14  & 3/5  & 0/0 & 2/10 & 5/14 & 2/7\\
%          Frequency:3      & 5/6  & 0/0  & 0/0  & 10/10  & 3/5  & 0/0 & 2/6 & 5/9 & 2/4 \\
%          Frequency:5      & 4/5  & 0/0  & 0/1  & 3/7  & 3/4    & 0/0 & 3/7 & 3/9 & 1/1\\
%          \midrule\midrule
% 		      {\bf Project} & {\bf Math} & {\bf Time} & {\bf Cli}  & {\bf  Jsoup} & {\bf JxPath} & {\bf  JacksonXml} & {\bf  Mockito}  &  {\bf  JacksonCore} & {\bf Total}  \\ 
% 	        \midrule
%           Frequency:2      &9/17 & 1/3  & 0/5  & 3/4  & 0/1  & 0/0 & 1/1 & 1/1 & 43/91\\
%           Frequency:3      & 10/15  & 2/3  & 0/2  & 1/2  & 0/0  & 0/0 & 1/1 & 1/1 & 42/64 \\
%           Frequency:5      & 9/19  & 2/3  & 1/2  & 2/5  & 0/2  & 0/0 & 1/1 & 1/2 & 32/68\\
% 		\bottomrule
% 		\end{tabular}
% 		\end{threeparttable}
% %	}

% \end{table*}

\begin{table}[!t]
\caption{Effects of Token-level fix with different frequent threshold}
	\label{tab:frequency}
\centering
\setlength\tabcolsep{3pt}
	\resizebox{0.50\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{l|c|c|c}
\toprule
\bf{Frequency} & \bf{2} & \bf{3} & \bf{5} \\ \midrule
Total      & 43/91 & 42/64 & 32/68          \\ \bottomrule      
\end{tabular}
\end{threeparttable}}
\end{table}

==> fig/table/sbflResult.tex <==
\begin{table}[!t]
\caption{Repair result comparison when using SBFL}
	\label{tab:sbfl_result}
\centering
\resizebox{1.0\columnwidth}{!}{
\setlength\tabcolsep{3pt}
\begin{threeparttable}
% \begin{tabular}{l|clc}
% \hline
% 			\toprule
% \bf Project & \multicolumn{1}{c|}{\bf  \tool{}} & \multicolumn{1}{l|}{\bf Project} & \bf \tool{} \\ \toprule
% Chart                          & \multicolumn{1}{c|}{4/4}                            & \multicolumn{1}{l|}{Gson}                           & 2/2                           \\
% Cli                            & \multicolumn{1}{c|}{1/3}                            & \multicolumn{1}{l|}{JacksonDataBind}                & 4/4                           \\
% Closure                        & \multicolumn{1}{c|}{3/5}                            & \multicolumn{1}{l|}{JSoup}                          & 2/2                           \\
% Codec                          & \multicolumn{1}{c|}{4/4}                            & \multicolumn{1}{l|}{Lang}                           & 2/2                           \\
% Compress                       & \multicolumn{1}{c|}{1/2}                            & \multicolumn{1}{l|}{Math}                           & 7/9                           \\ \hline
% \midrule
% Total                          & \multicolumn{3}{c}{30/37}                                                                                                                 \\ \midrule
% P(\%)                          & \multicolumn{3}{c}{81.1\%}                                                                        \\ \bottomrule
% \end{tabular}
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\bf{} & \bf{SimFix} & \bf{TBar} & \bf{TransplantFix} & \bf{Recoder} & \cellcolor{lightgray}\bf{\tool{}} &\cellcolor{lightgray}\bf{\combine{}}\\ \midrule
Total     & 36/81           & 50/131        & 44/137                 & 70/140           & \cellcolor{lightgray}\bf{31/37}    & \cellcolor{lightgray}\bf{90/236}          \\
Precision (\%)     & 44.4            & 38.2          & 32.1                   & 50.0            & \cellcolor{lightgray}\bf{ 83.8}   & \cellcolor{lightgray}\bf{38.1}   \\ \bottomrule      
\end{tabular}
\end{threeparttable}
}
\end{table}

==> fig/table/subject.tex <==
\begin{table}[t]
	\caption{Details of the experimental benchmarks}
	\label{tab:subject}
	\centering
    \resizebox{1.00\textwidth}{!}{
	\begin{tabular}{c|lrrr|c|lrrr}
		\toprule
		\textbf{Ver.} & \textbf{Project} & \textbf{\#Bugs} & \textbf{\#kLoc} & \textbf{Description} & \textbf{Ver.} & \textbf{Project} & \textbf{\#Bugs} & \textbf{\#kLoc} & \textbf{Description}\\
		\midrule
        \multirow{6}{*}{v1.2} &
        \textbf{Mockito} & 38 & 22 & Mocking framework for unit tests& 
        \multirow{9}{*}{v2.0} & commons-collections  (\textbf{Collections}) &  4 & 60 & Java library of data structures\\
        
        & closure-compiler (\textbf{Closure}) & 131 & 90 & JavaScript checker and optimizer& & commons-compress (\textbf{Compress}) & 47 & 25 & A library of file (de)compress\\
        
        & jfreechart (\textbf{Chart}) & 26 & 96 & A Java library for drawing chart & & commons-csv (\textbf{Csv}) & 16 & 4& Reading and writing CSV files\\
        
        & commons-lang (\textbf{Lang}) & 64 & 22 & Apache Java utility classes& & \textbf{Gson} & 18 & 24 & Java (de)serialization library\\
        
        & commons-math (\textbf{Math}) & 106 & 85 & A library for mathematics& & jackson-core (\textbf{JacksonCore}) & 26 & 33 & Core part of Jackson (basic APIs)\\
		
        & joda-time (\textbf{Time}) & 26 & 28 & Java date and time library& & jackson-databind (\textbf{JacksonDatabin}) & 112 & 9 & General data-binding package\\ \cline{1-5}
        
        \multirow{3}{*}{v2.0}
        & closure-compiler (\textbf{Closure}) & 43 & 90 & JavaScript checker and optimizer& & jackson-dataformat-xml (\textbf{JacksonXml}) & 6 & 47 & Reading and writing XML files\\
        
        & commons-cli(\textbf{Cli}) & 39 & 5& A library of processing command lines& & \textbf{Jsoup} & 93 & 15 & A Java HTML parser\\
        
        & commons-codec(\textbf{Codec}) &  18  &  11 & Common encoders and decoders& & commons-jxpath (\textbf{JxPath})  & 22 & 25&  The interpreter of language XPath\\
		
		% \midrule
		% \textbf{Total} & 835 & &  \\
		\bottomrule
	\end{tabular}
 }
\end{table}

==> table/combine.tex <==
\begin{table*}[!t]
\caption{Sources of correct patches}
	\label{tab:combine_sources}
\centering
\resizebox{\columnwidth}{!}{
\setlength\tabcolsep{3pt}
\begin{threeparttable}
\begin{tabular}{l|c|c|c|c|c}
\toprule
\bf{} & \bf{SimFix} & \bf{TBar} & \bf{TransplantFix} & \cellcolor{lightgray}\bf{\tool{}} \\
\midrule
Number     & 12           & 39        & 23           & \cellcolor{lightgray}\bf{39}           \\
Ratio (\%)     & 9.6            & 31.2          & 18.4   & \cellcolor{lightgray}\bf{40.8}      
\\ \bottomrule      
\end{tabular}
\end{threeparttable}
}
\end{table*}

==> table/deprecated.tex <==
\begin{table*}[!t]
	\centering
	%\scriptsize
	\setlength\tabcolsep{2pt}
%	\caption{Comparing \toolname against the state-of-the-art APR tools.}
	\label{tab:comparisonPerfect}
%	\resizebox{1.00\linewidth}{!}
%    {
    	\begin{threeparttable}
% 			\begin{tabular}{l|c|c|c|c|c}
% 			\toprule
% 		      {\bf Project} & {\bf  Recoder} &  {\bf  TBar} & {\bf SimFix}  & {\bf TransplantFix}   & {\cellcolor{lightgray}{\bf Repatt}}  \\ 
% 	        \hline
%  Chart          & 8/14  & 9/14  & 4/8  & 8/16    & \cellcolor{lightgray}{\bf 9/14}\\
%  Cli            & 3/3  & 1/7  & 0/4    & -        & \cellcolor{lightgray}{\bf 9/14}\\
%  Closure        & 17/38 & 8/17 & 7/13  & 7/11   & \cellcolor{lightgray}{\bf 9/14}\\
%  Codec          & 2/2  & 2/6  & 0/2     & -     & \cellcolor{lightgray}{\bf 9/14}\\
%  Collections    & 0/0  & 0/1  & 0/1     & -    & \cellcolor{lightgray}{\bf 9/14}\\
%  Compress       & 3/9  & 1/13  & 0/6    & -    & \cellcolor{lightgray}{\bf 9/14}\\
%  Csv            & 4/4  & 1/5  & 0/2    & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  Gson           & -    & -     & -     & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  JacksonCore    & 0/4  &  0/6  & 0/0    & -     & \cellcolor{lightgray}{\bf 9/14}\\
%  JacksonDatabind& 0/0  & 0/0  & 0/0    & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  JacksonXml     & -    & -    & -      & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  Jsoup          & 7/13  & 3/7  & 1/5  & -      & \cellcolor{lightgray}{\bf 9/14}\\
%  JxPath         & 0/4  & 0/0  & 0/0    &-      & \cellcolor{lightgray}{\bf 9/14}\\
%  Lang           & 9/15  & 5/14  & 9/13   & 8/15   & \cellcolor{lightgray}{\bf 9/14}\\
%  Math          & 15/30 & 18/36  & 14/26  & 20/41   & \cellcolor{lightgray}{\bf 9/14}\\
%  Mockito        & 2/2  & 1/2  & 0/0   & 1/2   & \cellcolor{lightgray}{\bf 9/14}\\
%  Time           & 2/2  & 1/3  & 1/1   & 3/6   & \cellcolor{lightgray}{\bf 9/14}\\
% 			\hline
% 	  Total   & 69/137  & 50/131  & 36/81  & 47/91   & \cellcolor{lightgray}{\bf 9/14} \\\hline
% P(\%)         & 50.4  & 38.2     & 44.4  & 51.6      & \cellcolor{lightgray}{11.1} \\
% 		\bottomrule
% 		\end{tabular}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\bf Project & \bf Recoder & \bf TBar & \bf SimFix & \bf TransplantFix & \bf SelfRepair & \bf CodeT5 & \bf CodeGen & \bf PLBART & \bf Repatt \\
Cli              & 3/-              & 1/7           & 0/1             & 4/8                    & 8/-                 & 2/3             & 4/5              & 2/3             & \cellcolor{lightgray}{\bf 3/9} \\
Codec            & 2/-              & 3/6           & 1/1             & 2/4                    & 8/-                 & 1/1             & 2/3              & 1/1             & \cellcolor{lightgray}{\bf 3/6} \\
Collections      & 0/-              & 0/0           & 0/0             & 0/0                    & 1/-                 & 0/0             & 1/1              & 0/0             & \cellcolor{lightgray}{\bf 0/0} \\
Compress         & 3/-              & 2/12          & 0/4             & 4/10                   & 7/-                 & 3/5             & 3/6              & 3/5             & \cellcolor{lightgray}{\bf 3/13}   \\
Csv              & 4/-              & 3/6           & 0/2             & 1/2                    & 1/-                 & 1/2             & 2/3              & 2/4             & \cellcolor{lightgray}{\bf 1/3} \\
Gson             & 0/-              & 1/4           & 2/2             & 1/2                    & 1/-                 & 0/0             & 0/0              & 0/0             & \cellcolor{lightgray}{\bf 2/3} \\
JacksonCore      & 0/-              & 0/5           & 0/2             & 1/6                    & 3/-                 & 3/3             & 2/3              & 2/2             & \cellcolor{lightgray}{\bf 2/7} \\
JacksonDatabind  & 0/-              & 2/17          & 1/10            & 7/20                   & 8/-                 & 4/7             & 3/6              & 2/4             & \cellcolor{lightgray}{\bf 10/18}  \\
JacksonXml       & -                & 0/1           & 0/0             & 0/0                    & 1/-                 & 0/0             & 0/0              & 0/0             & \cellcolor{lightgray}{\bf 0/0} \\
Jsoup            & 7/-              & 7/17          & 1/2             & 3/8                    & 6/-                 & 4/6             & 5/7              & 4/5             & \cellcolor{lightgray}{\bf 3/13}   \\
JxPath           & 0/-              & 0/0           & 0/0             & 2/7                    & 1/-                 & 0/0             & 0/1              & 0/1             & \cellcolor{lightgray}{\bf 0/5} \\
Mockito          & 2/-              & 3/3           & 1/2             & 3/3                    & 3/-                 & 4/5             & 3/4              & 2/3             & \cellcolor{lightgray}{\bf 1/2} \\
Closure          & 23/-             & 17/25         & 7/15            & 10/22                  & 20/-                & 7/10            & 10/13            & 6/11            & \cellcolor{lightgray}{\bf 11/12}  \\
Chart            & 10/-             & 11/13         & 8/16            & 6/10                   & 7/-                 & 4/4             & 7/7              & 4/4             & \cellcolor{lightgray}{\bf 6/7} \\
Lang             & 10/-             & 13/18         & 8/15            & 4/10                   & 10/-                & 6/8             & 5/5              & 4/4             & \cellcolor{lightgray}{\bf 6/11}   \\
Math             & 19/-             & 22/34         & 20/33           & 12/25                  & 21/-                & 12/14           & 12/14            & 13/16           & \cellcolor{lightgray}{\bf 14/25}  \\
Time             & 3/-              & 2/5           & 3/6             & 1/3                    & 3/-                 & 1/1             & 2/2              & 2/2             & \cellcolor{lightgray}{\bf 1/3} \\
Total            &                  &               &                 &                        &                     &                 &                  &                 & \cellcolor{lightgray}{\bf }       \\
P(\%)            &                  &               &                 &                        &                     &                 &                  &                 & \cellcolor{lightgray}{\bf }      
\end{tabular}
		\end{threeparttable}


\end{table*}

==> table/frequency.tex <==
% \begin{table*}[!t]
% \caption{Effects of Token-level fix with different frequent threshold\jcom{@Zijie, add frequency:5.}}
% 	\label{tab:frequency}
% 	\centering
% 	%\scriptsize
% 	\setlength\tabcolsep{3pt}
% %	\resizebox{1.00\linewidth}{!}
% %    {
%     	\begin{threeparttable}
% 			\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% 			\toprule
% 		      {\bf Project} & {\bf Chart} & {\bf Gson} & {\bf  Csv}  & {\bf  Closure} & {\bf Codec} & {\bf Collections} & {\bf Compress}  &{\bf JacksonDatabind } & {\bf Lang }   \\ 
% 	        \midrule
%          Frequency:2      & 6/8  & 0/0  & 0/1  & 10/14  & 3/5  & 0/0 & 2/10 & 5/14 & 2/7\\
%          Frequency:3      & 5/6  & 0/0  & 0/0  & 10/10  & 3/5  & 0/0 & 2/6 & 5/9 & 2/4 \\
%          Frequency:5      & 4/5  & 0/0  & 0/1  & 3/7  & 3/4    & 0/0 & 3/7 & 3/9 & 1/1\\
%          \midrule\midrule
% 		      {\bf Project} & {\bf Math} & {\bf Time} & {\bf Cli}  & {\bf  Jsoup} & {\bf JxPath} & {\bf  JacksonXml} & {\bf  Mockito}  &  {\bf  JacksonCore} & {\bf Total}  \\ 
% 	        \midrule
%           Frequency:2      &9/17 & 1/3  & 0/5  & 3/4  & 0/1  & 0/0 & 1/1 & 1/1 & 43/91\\
%           Frequency:3      & 10/15  & 2/3  & 0/2  & 1/2  & 0/0  & 0/0 & 1/1 & 1/1 & 42/64 \\
%           Frequency:5      & 9/19  & 2/3  & 1/2  & 2/5  & 0/2  & 0/0 & 1/1 & 1/2 & 32/68\\
% 		\bottomrule
% 		\end{tabular}
% 		\end{threeparttable}
% %	}

% \end{table*}

\begin{table*}[!t]
\caption{Effects of Token-level fix with different frequent threshold}
	\label{tab:frequency}
\centering
\setlength\tabcolsep{3pt}
	\resizebox{0.50\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{l|c|c|c}
\toprule
\bf{Frequency} & \bf{2} & \bf{3} & \bf{5} \\ \midrule
Total      & 43/91 & 42/64 & 32/68          \\ \bottomrule      
\end{tabular}
\end{threeparttable}}
\end{table*}

==> table/patterns.tex <==
\begin{table*}[htb]
\caption{Average number of trees and leaf nodes of each project}
\label{tab:patterns}
\centering
\resizebox{1.0\columnwidth}{!}{
\setlength\tabcolsep{3pt}
\begin{tabular}{|c|c||c|}
\toprule
Projects &  Average amount of trees & Average amount of leaf nodes \\
\midrule
Chart & 9891.19 & 2650236.25\\
Closure & 14263.42 & 3273520.48 \\
Lang & 2589.77 & 736499.64 \\
Math & 6353.01 & 2660681.53 \\
Mockito  & 1830.69 & 193381.38\\
Cli  & 420.25 & 59161.38\\
Codec & 825.75 & 339805.33\\
Collections & 3412.00 & 567026.00\\
Compress & 2877.39 & 745581.0\\
Csv  & 313.42 & 62076.08\\
Gson & 1602.89 & 273406.33\\
JacksonCore & 1897.64 & 506916.71\\
JacksonDatabind  & 6705.36 & 1358046.62\\
JacksonXml & 856.25 & 89513.25\\
Jsoup & 1843.66 & 362774.26\\
JxPath & 2366.33 & 519456.78\\
\midrule
\textbf{Average} & 5961.11 & 1546656.45\\
\bottomrule
\end{tabular}
}
\end{table*}

==> table/subject.tex <==
\begin{table*}[t]
	\caption{Details of the experimental benchmarks}
	\label{tab:subject}
	\centering
    \resizebox{1.00\textwidth}{!}{
	\begin{tabular}{c|lrrr|c|lrrr}
		\toprule
		\textbf{Ver.} & \textbf{Project} & \textbf{\#Bugs} & \textbf{\#kLoc} & \textbf{Description} & \textbf{Ver.} & \textbf{Project} & \textbf{\#Bugs} & \textbf{\#kLoc} & \textbf{Description}\\
		\midrule
        \multirow{6}{*}{v1.2} &
        \textbf{Mockito} & 38 & 22 & Mocking framework for unit tests& 
        \multirow{9}{*}{v2.0} & commons-collections  (\textbf{Collections}) &  4 & 60 & Java library of data structures\\
        
        & closure-compiler (\textbf{Closure}) & 131 & 90 & JavaScript checker and optimizer& & commons-compress (\textbf{Compress}) & 47 & 25 & A library of file (de)compress\\
        
        & jfreechart (\textbf{Chart}) & 26 & 96 & A Java library for drawing chart & & commons-csv (\textbf{Csv}) & 16 & 4& Reading and writing CSV files\\
        
        & commons-lang (\textbf{Lang}) & 64 & 22 & Apache Java utility classes& & \textbf{Gson} & 18 & 24 & Java (de)serialization library\\
        
        & commons-math (\textbf{Math}) & 106 & 85 & A library for mathematics& & jackson-core (\textbf{JacksonCore}) & 26 & 33 & Core part of Jackson (basic APIs)\\
		
        & joda-time (\textbf{Time}) & 26 & 28 & Java date and time library& & jackson-databind (\textbf{JacksonDatabin}) & 112 & 9 & General data-binding package\\ \cline{1-5}
        
        \multirow{3}{*}{v2.0}
        & closure-compiler (\textbf{Closure}) & 43 & 90 & JavaScript checker and optimizer& & jackson-dataformat-xml (\textbf{JacksonXml}) & 6 & 47 & Reading and writing XML files\\
        
        & commons-cli(\textbf{Cli}) & 39 & 5& A library of processing command lines& & \textbf{Jsoup} & 93 & 15 & A Java HTML parser\\
        
        & commons-codec(\textbf{Codec}) &  18  &  11 & Common encoders and decoders& & commons-jxpath (\textbf{JxPath})  & 22 & 25&  The interpreter of language XPath\\
		
		% \midrule
		% \textbf{Total} & 835 & &  \\
		\bottomrule
	\end{tabular}
 }
\end{table*}
